Reduced Basis, Embedded Methods and Parametrized Levelset Geometry

In this chapter we examine reduced order techniques for geometrical parametrized heat exchange systems, Poisson, and flows based on Stokes, steady and unsteady incompressible Navier-Stokes and Cahn-Hilliard problems. The full order finite element methods, employed in an embedded and/or immersed geometry framework, are the Shifted Boundary (SBM) and the Cut elements (CutFEM) methodologies, with applications mainly focused in fluids. We start by introducing the Nitsche's method, for both SBM/CutFEM and parametrized physical problems as well as the high fidelity approximation. We continue with the full order parameterized Nitsche shifted boundary variational weak formulation, and the reduced order modeling ideas based on a Proper Orthogonal Decomposition Galerkin method and geometrical parametrization, quoting the main differences and advantages with respect to a reference domain approach used for classical finite element methods, while stability issues may overcome employing supremizer enrichment methodologies. Numerical experiments verify the efficiency of the introduced ``hello world'' problems considering reduced order results in several cases for one, two, three and four dimensional geometrical kind of parametrization. We investigate execution times, and we illustrate transport methods and improvements. A list of important references related to unfitted methods and reduced order modeling are [11, 8, 9, 10, 7, 6, 12].

==> install-getnonfreefonts <==
#! /usr/bin/env texlua
--*- Lua -*-
--  -- pretend that this is a binary file.
-- Web browsers shall download the file, not display it.

-- Copyright (C) 2009-2015 Reinhard Kotucha <kotucha@tug.org>
--
-- You may freely use, modify and/or distribute this file.

installer_release='2018-06-04'

----------------------------------------------------------------
-- The following variables are only used for TeX systems whose
-- file system layout is not identical to that created by the
-- TeX Live installer.  This is usually the case for TeX systems
-- shipped with Linux/Unix distributions (binaries for a single 
-- platform only, and texmf* in /usr/share).
--
-- By default we install in /usr/local in order not to interfere
-- with the package manager of your Linux/Unix distribution.
--
-- These variables have no effect if you have a TeX Live system 
-- from http://texlive.org .

BINDIR='/usr/local/bin'
MANDIR='/usr/local/share/man/man1'

----------------------------------------------------------------
-- You don't have to change anything below this line.
----------------------------------------------------------------

--> !!BEGIN-INSERTED-FILES!!

-- Date: Fri Jun  2 00:18:33 2017 UTC

script=[[
#!/usr/bin/env perl

# $Id: $

# Copyright (C) 2006-2017 Reinhard Kotucha <reinhard.kotucha@web.de>
# 
# You may freely use, modify, and/or distribute this file.

my $revision='2017-06-02';

use Getopt::Long;
$Getopt::Long::autoabbrev=0;
Getopt::Long::Configure ("bundling");

my $getfont_url='https://www.tug.org/~kotucha/getnonfreefonts/getfont.pl';
my $banner="This is getnonfreefonts, revision $revision.\n\n";

# messages

my $usage = <<'ENDUSAGE';
Usage:
    getnonfreefonts --sys|--user [options] [font1] [font2] ...

    getnonfreefonts --sys installs fonts in $TEXMFLOCAL.
    getnonfreefonts --user installs fonts in $TEXMFHOME.

    In nearly all cases you should use getnonfreefonts --sys.
    For special cases see 

        http://tug.org/texlive/scripts-sys-user.html

    Options:

        -a|--all        Install all fonts.

        -d|--debug      Provide additional messages for debugging.

        -f|--force      Install fonts even if they are installed already.

        -h|--help       Print this message.

        -l|--lsfonts    List all fonts available.

        -r|--refreshmap Refresh map file.

        -H|--http       Use http instead of ftp (see manual).

        --version       Print version number.

ENDUSAGE


my $sys_user_err = <<'EOF';
ERROR: You have to invoke getnonfreefonts with either --sys or --user.

In nearly all cases you should use getnonfreefonts --sys.
For special cases see 

   http://tug.org/texlive/scripts-sys-user.html

EOF


# system specific stuff

my %sys=(
  w32     => 0,
  dirsep  => '/',
  pathsep => ':',
  exe     => '',
  dollar  => '\$',
  nulldev => '>/dev/null 2>/dev/null' 
    );

if ($^O=~/^MSWin(32|64)/i) {
  %sys=(
    w32     => 1,
    dirsep  => '\\',
    pathsep => ';',
    exe     => '.exe',
    dollar  => '$',
    nulldev => '>NUL 2>NUL' 
      );
}

# GetOptions removes optional arguments from @ARGV.
# We have to create a new array because assignments create references.

my @ARGS;
foreach my $arg (@ARGV) {
  push (@ARGS, $arg);
}

$opt_lsfonts=0;
$opt_force=0;
$opt_sys=0;
$opt_user=0;

$done=GetOptions 
    "all|a",
    "debug|d",
    "force|f",
    "help|h",
    "http|H",
    "lsfonts|l",
    "refreshmap|r",
    "verbose|v",
    "version|V",
    "sys|s",
    "user|u";

@allpackages=@ARGV;


# ANSI colors

my @supported_terminals=(
  'Eterm', 'ansi', 'color-xterm', 'con132x25', 'con132x30',
  'con132x43', 'con132x60', 'con80x25', 'con80x28', 'con80x30',
  'con80x43', 'con80x50', 'con80x60', 'cons25', 'console', 'cygwin',
  'dtterm', 'gnome', 'gnome-256color', 'konsole', 'kterm', 'linux',
  'linux-c', 'mach-color', 'mlterm', 'putty', 'rxvt', 'rxvt-cygwin',
  'rxvt-cygwin-native', 'rxvt-unicode', 'screen', 'screen-bce',
  'screen-w', 'screen.linux', 'vt100', 'xterm', 'xterm-256color',
  'xterm-color', 'xterm-debian'
    );

my $term_supported=0;

if ($ENV{'TERM'}) {
  foreach my $terminal (@supported_terminals) {
    if ($ENV{'TERM'} eq $terminal) {
      $term_supported=1;
    }
  }
}

sub colored {
  my $text=shift;
  my $color=shift;

  my $esc="\e[";
  my $restore="\e[0m";

  %colors=(
    red   => '00;31m',
    green => '00;32m'
      );

  if ($term_supported and -t 'STDOUT') {
    return "${esc}$colors{$color}${text}${restore}";
  } else {
    return $text;
  }
}

# messages

my $msglen=0;

sub msg {
  my $message=shift;
  $msglen=length($message);
  print $message;
}

sub status {
  my $status=shift;
  my $color=shift;

  
  my $spaces=79-2-$msglen-length($status);
  $spaces=1 if ($spaces < 1);
  print ' ' x $spaces;
  print ('[' . colored($status, $color) . "]\n");
}

sub debug_msg {
  my $message=shift;
  if ($opt_debug) {
    print STDERR "DEBUG: $message\n";
  }
}

# kpathsea stuff

sub var_value {
  my $var=shift;
  my $ret;

  $ret=`kpsewhich --var-value=$var`;
  chomp($ret);
  return $ret;
}

sub expand_var {
  my $var=shift;
  my $ret;
  my $dollar=$sys{'dollar'};
  $ret=`kpsewhich --expand-var=$dollar$var`;
  chomp($ret);
  return $ret;
}

sub expand_braces {
  my $var=shift;
  my $pathsep;
  my $retstring;
  my @retlist;
  if ($sys{'w32'}) {
    open KPSEWHICH, 'kpsewhich --expand-braces=$'  . "$var |";
    $pathsep=';';
  } else {
    open KPSEWHICH, 'kpsewhich --expand-braces=\$' . "$var |";
    $pathsep=':';
  }
  $retstring=(<KPSEWHICH>);
  close KPSEWHICH;
  chop $retstring;
  @retlist=split $pathsep, $retstring;
  if ($opt_debug) {
    my $index=0;
    foreach my $entry (@retlist) {
	    debug_msg "$var\[$index\]: '$entry'.";
	    ++$index;
    }
    debug_msg "Extracting the first element of the list ($var\[0\]):";
    debug_msg "$var\[0\]='$retlist[0]'.";
  }
  return "$retlist[0]";
}

sub get_tmpdir {
  if ($opt_debug) {
    for my $var (qw(TMPDIR TEMP)) {
      if (defined $ENV{$var}) {
        debug_msg "Environment variable $var='$ENV{$var}'.";
      } else {
        debug_msg "Environment variable $var not set.";
      }
    }
  }
  # get TMPDIR|TEMP environment variable, use /tmp as fallback.

  my $SYSTMP=undef;
  $SYSTMP||=$ENV{'TMPDIR'};
  $SYSTMP||=$ENV{'TEMP'};
  $SYSTMP||='/tmp';
  return "$SYSTMP";
}

sub which {
  my $prog=shift;
  my @PATH;
  my $PATH=$ENV{'PATH'};
  if ($sys{'w32'}) {
    my @PATHEXT=split ';', $ENV{'PATHEXT'};
    push @PATHEXT, '';  # if argument contains an extension
    @PATH=split ';', $PATH;
    for my $dir (@PATH) {
      $dir=~s/\\/\//g;
      for my $ext (@PATHEXT) {
        if (-f "$dir/$prog$ext") {
          return "$dir/$prog$ext";
        }
      }
    }
  } else {
    @PATH=split ':', $PATH;
    for my $dir (@PATH) {
      if (-x "$dir/$prog") {
        return "$dir/$prog";
      }
    }
  }
  return 0;
}

sub show_path {
  my @PATH;
  @PATH=split($sys{'pathsep'}, $ENV{'PATH'});
  my $index=0;
  
  foreach my $dir (@PATH) {
    debug_msg "PATH\[$index\]: '$dir'.";
    ++$index;
  }
}

sub signals {
  # Signals supposed to be supported by Windows are derived from the
  # sources of the Microsoft C runtime library.  It's a matter of fact
  # that not everything described there really works.  Furthermore,
  # the behavior depends heavily on the version of Windows you are
  # using.  Don't expect too much.
  my @signals;
  my @common_signals=qw(INT ILL FPE SEGV TERM ABRT);
  my @signals_UNIX=qw(QUIT BUS PIPE);
  my @signals_Win32=qw(BREAK);

  if ($sys{'w32'}) {
    @signals=(@common_signals, @signals_Win32);
  } else {
    @signals=(@common_signals, @signals_UNIX);
  }
  return @signals;
}


sub check_tmpdir{
  my $SYSTMP=shift;
  die "! ERROR: The temporary directory '$SYSTMP' doesn't exist.\n"
      unless (-d "$SYSTMP");

  die "! ERROR: The temporary directory '$SYSTMP' is not writable.\n"
      unless (-w "$SYSTMP");
}

sub check_installroot {
  my ($INSTALLROOTNAME, $INSTALLROOT)=@_;
  mkdir "$INSTALLROOT" unless (-d "$INSTALLROOT");

  die "! ERROR: The variable $INSTALLROOTNAME is not set.\n"
      unless length ("$INSTALLROOT") > 0;
  
  die "! ERROR: The install directory '$INSTALLROOT' doesn't " .
      "exist.\n" .
      "         If this is the correct path, please create " .
      "this directory manually.\n" 
      unless (-d "$INSTALLROOT");
  
  die "! ERROR: The install directory '$INSTALLROOT' is not writable.\n"
      unless (-w "$INSTALLROOT");
}

sub check_binary {
  my $binary=shift;
  if ($opt_debug) {
    debug_msg "Search for $binary in PATH:";
    my $binary=which "$binary";
    debug_msg "Found '$binary'.";
  }
}


### main ####

debug_msg "getnonfreefonts rev. $revision.";

debug_msg ("argv[0]: '$0'");
my $nargs=@ARGS+0;
for (0..$#ARGS) {
  my $i=$_;
  my $arg=$ARGS[$i];
  $i++;
  debug_msg ("argv[$i]: '$arg'");
}

debug_msg("opt_sys=$opt_sys");
debug_msg("opt_user=$opt_user");

show_path() if ($opt_debug);

check_binary 'kpsewhich';

# Determine INSTALLROOT.

$INSTALLROOTNAME=($opt_sys)? 'TEXMFLOCAL':'TEXMFHOME';

$INSTALLROOT=expand_braces "$INSTALLROOTNAME";

# Remove trailing exclamation marks and double slashes.

debug_msg "Removing leading \"!!\" and trailing \"//\" " . 
    "and set INSTALLROOT:";

$INSTALLROOT=~s/^!!//;
$INSTALLROOT=~s/\/\/$//;

debug_msg "INSTALLROOT='$INSTALLROOT'.";

my $SYSTMP=get_tmpdir;

debug_msg "Internal variable SYSTMP set to '$SYSTMP'.";

$^W=1 if $opt_debug;

unless ($done) {
  print STDERR "\n$banner$usage";
  exit 1;
}

if ($opt_version) {
  print "$revision\n";
  exit 0;
}

if ($opt_sys and $opt_user) {
  print STDERR "$sys_user_err";
  exit 1;
}

if ($opt_help) {
  print ($banner);
  print ($usage);

  if ($opt_sys or $opt_user) {
    print <<"ENDUSAGE";
    Directories:
       temporary: '$SYSTMP/getfont-<PID>'
       install:   '$INSTALLROOT'

ENDUSAGE
  } else {
    print "$sys_user_err";
  }
  exit 0;
}

  
unless ($opt_sys or $opt_user) {
  print "$sys_user_err";
  exit 1;
}

if ($opt_sys and $opt_user) {
  print "$sys_user_err";
  exit 1;
}


check_tmpdir $SYSTMP;
check_installroot "$INSTALLROOTNAME", "$INSTALLROOT";

my $tmpdir="$SYSTMP" . $sys{'dirsep'} . "getfont-$$";
debug_msg "Internal variable tmpdir set to '$tmpdir'.";

mkdir "$tmpdir" or die "ERROR: Can't mkdir '$tmpdir'.";
chdir "$tmpdir" or die "ERROR: Can't cd '$tmpdir'.";

#install_signal_handlers $SYSTMP, $tmpdir;

sub remove_tmpdir {
  debug_msg "Executing Signal Handler:";
  chdir "$SYSTMP" or die "! ERROR: Can't cd '$SYSTMP'.\n";
  opendir TMPDIR, "$tmpdir" 
      or print "! ERROR: Can't read directory '$tmpdir'.\n";
  my @alltmps=readdir TMPDIR;
  closedir TMPDIR;
  foreach my $file (@alltmps) {
    next if $file=~/^\./;
    unlink "$tmpdir/$file";
    debug_msg "unlink '$tmpdir/$file'.";
  }
  rmdir "$tmpdir" or die 
      "! ERROR: Can't remove directory '$tmpdir'.\n";
  debug_msg "rmdir  '$tmpdir'.";
}

foreach my $signal (signals) {
  $SIG{"$signal"}=\&remove_tmpdir;
}
debug_msg 
    "Signal handlers installed. Don't expect too much on Windows.";

my $TLROOT=expand_var 'SELFAUTOPARENT'; ### only used on Windows,
                                        ### hence no portability
                                        ### problem
my $BINDIR=expand_var 'SELFAUTOLOC';

my $has_wget=0;
my $WGET;

if ($sys{'w32'}) { ## wget is shipped with TL.
  $has_wget=1;
  if (-f "$TLROOT\\tlpkg\\installer\\wget\\wget.exe") {
    # TL-2008+
    $WGET="$TLROOT\\tlpkg\\installer\\wget\\wget.exe";
  } elsif (-f "$BINDIR\\wget.exe") {
    # TL-2005...TL-2007
    $WGET="$BINDIR\\wget.exe";
  } else {
    die "ERROR: No wget binary found.\n";
  }
} elsif (which "wget") {
  $WGET='wget';
  $has_wget=1; ## wget is in PATH.
}


debug_msg "No wget binary found on your system, trying curl." 
    unless ($has_wget);

if ($has_wget) {
  debug_msg "Running '$WGET $getfont_url'.";
  system ("$WGET", "$getfont_url") == 0 
      or die "! Error: Can't execute wget.\n";
} else {
  debug_msg "Running 'curl -O $getfont_url'.";
  system ('curl', '-O', "$getfont_url") == 0 
      or die "! Error: Can't execute curl.\n";
}

# Download the fonts.

my @getfont=('perl', "./getfont.pl");
push @getfont, "--installroot=$INSTALLROOT";
push @getfont, '--lsfonts' if $opt_lsfonts;
push @getfont, '--force' if $opt_force;
push @getfont, '--debug' if $opt_debug;
push @getfont, '--verbose' if $opt_verbose;
push @getfont, '--sys' if $opt_sys;
push @getfont, '--refreshmap' if $opt_refreshmap;
push @getfont, '--all' if $opt_all;
push @getfont, '--http' if $opt_http;
if ($has_wget) {
  push @getfont, "--wget_bin=$WGET";
} else {
  push @getfont, '--use_curl';
}
push @getfont, @allpackages;

my $getfont_cmd=join " ", @getfont;

debug_msg "Running '$getfont_cmd'.";

system @getfont;

# Evaluate the exit status.  It will be 2 if something had been
# installed and in this case we need to run texhash/updmap.

my $exit_code=$?;
my $exit_status=int($exit_code/256);

my $has_updmap_user=0;
if (-f var_value('SELFAUTOLOC').'/updmap-user'.$sys{'exe'}) {
  $has_updmap_user=1;
}

if ($opt_sys) {	     
  debug_msg "Info: Execute updmap-sys if exit status is 2.";
} else {
  if ($has_updmap_user) {
    debug_msg "Info: Execute updmap-user if exit status is 2.";
  } else {
    debug_msg "Info: Execute updmap if exit status is 2.";
  }
}

debug_msg "Exit status of getfont.pl is $exit_status.";

if ($exit_status==2) {
  print "\n";
  msg "Running 'mktexlsr $INSTALLROOT $sys{'nulldev'}' ...";
#  if ($sys{'w32'}) {
    my $ret=system "mktexlsr $INSTALLROOT $sys{'nulldev'}";
#  } else {
#    my $ret=system "mktexlsr $INSTALLROOT >/dev/null 2>/dev/null";
#  }
  
  $ret ? status 'failed', 'red' : status 'done', 'green';
   
  
  my $updmap_command;
  if ($has_updmap_user) {
    $updmap_command=($opt_sys)? 'updmap-sys':'updmap-user';
  } else {
    $updmap_command=($opt_sys)? 'updmap-sys':'updmap';
  }
  @updmap=("$updmap_command");
  push @updmap, '--quiet' unless $opt_verbose;
  print "\n";
  msg "Updating map files ($updmap_command). Be patient...";
  system @updmap;
  
  $? ? status('failed', 'red') : status('done', 'green');
}

remove_tmpdir;

__END__

# Local Variables:
#  mode: Perl
#  perl-indent-level: 2
#  indent-tabs-mode: nil
#  coding: utf-8-unix
# End:
# vim:set tabstop=2 expandtab:
]]

man=[[
.TH getnonfreefonts 1 "May 2017" "TeX Live" "TeX Live"
.SH NAME
getnonfreefonts \- download and install fonts which cannot be
distributed on a CD/DVD because the license doesn't allow to charge
money for the distribution.

.SH SYNOPSIS

.BI "getnonfreefonts --sys [" options "] [" font1 "] [" font2 "] [" font... ]
.sp
.BI "getnonfreefonts --user [" options "] [" font1 "] [" font2 "] [" font... ]

In nearly all cases you should use getnonfreefonts --sys.  For special cases see 
.br
    http://tug.org/texlive/scripts-sys-user.html
.br

.SH DESCRIPTION
Some font suppliers provide fonts which can be used freely but they
disallow that money is charged for the distribution.  Hence, for
distributions on CD or DVD it is usually impossible to include
these fonts.

.B "getnonfreefonts"
downloads and installs these fonts.

.B "getnonfreefonts --sys" 
installs files to $TEXMFLOCAL
and
.B "getnonfreefonts --user"
installs files to $TEXMFHOME

.BI "getnonfreefonts"
downloads and executes a helper script each time it is invoked.  This
script is not installed permanently on your system and only exists in
a temporary directory while
.BI "getnonfreefonts"
is running.  It allows 
.BI "getnonfreefonts"
to be aware of updates and new fonts.

Run
.B "getnonfreefonts --sys --lsfonts"
or
.B "getnonfreefonts --user --lsfonts"
to get a list of supported fonts.

.SH OPTIONS

.TP
.BR "-a" , " --all"
.rg
Install all fonts.

.TP
.BR "-d" , " --debug"
.rg
Provide additional messages for debugging.  These messages are sent to
STDERR.

.TP
.BR "-f" , " --force"
.rg
Install fonts even if they are installed already.

.TP
.BR "-h" , " --help"
.rg
Print a help message.  Nothing is installed but the directories where
the fonts will be installed and the temporary directory are shown.
.BI "<" PID ">" 
will be replaced by the process ID of the current
process. 

.TP
.BR "-H" , " --http"
.rg
Use HTTP instead of FTP.  This is useful if you are behind a firewall
which is blocking FTP.  However, you can't install fonts which are on
FTP servers.  Currently this is only "Adobe Euro".

.TP
.BR "-l" , " --lsfonts"
.rg
List all available fonts and tell whether they are installed already. 

.TP
.BR "-r" , " --refreshmap"
.rg
Register 
.B map 
files for already installed fonts and run 
.B updmap. 
This is needed after upgrading TeX Live to a newer release.

.TP
.BR "-V", " --version"
.rg
Print version number.

.SH REQUIREMENTS
On Unix systems
.BR "unzip"
and either
.BR "wget"
or 
.BR "curl"
must exist.

.SH BUGS
Please send bug reports to Reinhard Kotucha <reinhard.kotucha@web.de>.
]]

manpdf=[[
JVBERi0xLjQKJcfsj6IKNSAwIG9iago8PC9MZW5ndGggNiAwIFIvRmlsdGVyIC9GbGF0ZURlY29k
ZT4+CnN0cmVhbQp4nO1Y227cyBF911c0FgGWE3habN4ZBAEcS4YUyLYiTQIH2n2ghq0ZZilyluRI
nn/YX8k/5lQ3u3nxyKsk+xj4Qcawu7q66tSpU/0zc7lgLv3r/64fT05vYrZpT1y2Ofn5RKiPrP+z
fmR/XmFBQj+sHk70HsFij8Wpz5OUrR5PhJ9w32er5xNnI7uqrh4aKR/qqmt/cMQPC7ZarP554nku
jyJsXuU4idbKz+yqoE9L+BKy1RpreKJXkMlIm3ySbEOrXFohwpALT69xjpzVm/NESqtPb1L4zdOQ
XF/6acLDhC39SO3++HZklYep31v9cE6/D1eG34EbsyWOJde5Gx27KfsXy2vamPjci9K0vyh3w5SW
3znPVVlnOcuqnBVV22VlyfTG522x3rJ1VlV1x+4ly4u2a4r7Bc51XS9w9p3MWV2xjL07Oz1bBPRz
kDp/P8PidbZvJeu2kpXFWlatXPy4+svJ0vjQ++zktWyr71UWuA50xIPEFf2Nu8xGIuWxSFMT4LKs
R5sQSV+4/TdcqFt4oevUa3Wm2u0FPECUR0m+c7ZZsxAJd0UoEDP2WFfayd5oEPEeFM7hYUiIyxPf
+Hfn1I26o4mMSHmahBSZoq64sjbNtIgC7iPTXgI8kenbf3z8dH17easzm/aZBRD6CN3ZdC5EzNNU
pA7yusB90iQQjsrTctkeWnbXHyfc3kgacEDbgKfekU/tKGrDcZ4Obr/yxzt725E1IbiwF3cIIOK4
LZeHkcnFq215L9oawPBaW5zzaTQ9H6UxuKQq0fMED32BTASvDzMg3RyJM6IX/z/OR+M8kBUiHnM3
sRF3LitWyawpD4wYZ521smWHes/abb0vc0b0MWcyBXQ+I+Z0oN33M1IILCk4TfsCk+zkusjM+a2U
Gh1+yr1wqMFt1+3+cHra7Te8HhCyOe3kQoTOl7LQ7Gacij0epPboJzk62ksAKMMep+26KXZdS9dS
4FqgibgiiBy+7R7LY/yBIMZj/jg7v313c3m9uvz0cRrvgULQdKJYU95t/SgVubN2v9uVhWxatmtq
XEIf+1Tkck7+xPzwLWeUB2RL87+IBViOyK/nzJjOIP5O0XtjQ5z5QJxqiYlJ0WaWws1OgXzZ4gCH
H9+5zTpN1f3ehJb4gFYYm7AeioUXRzxOY6cd9wDBoyAS1k5DJmA8TGxjQKSSvofivprcFSD8JOEi
CIa+1RM+ORFy36JeYQ/7dQNgF7Jayze0Kkx4NOk+ZH3SUGNf72qppb47Y/iueyolBj216FjRIhN7
RO7Aisdd3bbFfYkmW6Nvr8t9rvpt2ydw3H0UdNB6U/Lz9YzXWzCIihIe235yh9aNLtuLh3asHtpv
umGsfNsN2hQkPAhMYKEbhE7NwARTwGN5FIbpsFxh3rFO/VKiwBGr363OP394f/Xp3dsr8npKYQLu
uX5o7jj1zfeO+zZuD1OfQrRg1zeYnruikRWhomPLNY527+KTEXuWXBGuq5PV7/+rvKVJYvqT1oLg
wHCO+XEq5YRkwxgq1FbOlxf4zFlDEGI728pyh0apyY3JDDzSFSAejeCiMlJYC1xSosbCU23O1db7
unR+Gh/p+/bIngDgfM7ZalsoSPg+1GA03E7JXKf3Bg6Qmu1TIXOdA6RT+MFAmAE8ok24xmNWyapD
xaEq0Z5wrUPbyUcVpbrC78o1EUGC+oE5NAj1hPAFBU43RlCwZ1c3WXNA1Tdy3dX4Hzi2lDMABjGP
DB+9AECVa6jMY7lGN4x9S7Ks2VdVUW1Uz6QCSUyBOJeKYJcB6CtJxdDqFC9TYbezykXLGXjuf2QP
PWahGNFbsnHKIf/DoWk/D/If8mMkdxrJ6ge23+WZQhxSYRqCwmuCtA965nmk3qFQwlHR8l4LoppH
yuRmX82Sgqjayen1iny5LFv9IfXiYzGhbu5bf5rZodNJ41eRYPTpr5/qe9ygACmAYcCzBFIppqQL
6qZT7c8EaDasIkdeKEYa5JOSHy+OMM4ym7IizeSua2r7zXSfCcdyCSTO5l0Pc7pVCJf9rGrn1Zka
pWl68HGZz31IRsx13Ic7OJHLUXvezCIJhwSh1RbPtdFSYaq1VJbnBTV1KMxH2bbZBnBVnR9myRY0
Bb0mTLXDZkMlCz5DFyXHIggXi31dOtZYhlJoQVDU2W5XZ+c3N/MweIHHvXQciodpKCKybgjzG6EA
qPqr9Ro4gTBZy3lMAkXQNvmXkyeFWV8JuLDiq9fJfQnPlHIFSRekBHznoRskHcb3ZBDa2xcNOIcJ
k6T+wLCIn20GwFIjs/ywiIwMn6sXgcFgAqvtfw4rhJI65FfYHkMJ3SQMtVC8boqq67uqARFfLEM/
BFWGzse62wIuurOae+iXCKp/rdFtzykkKXvZ6KeZXukXSM/9JAyQRQqdHmkOAX2imyztOdbHFAi3
9eJ7xS1+Yvm7mk+I0Pg233/U3+yECVrpv1xfns1l2Shnzp+mocNN40SYpmdu08hdma0pFgd1V4w5
awSPXZ4RzdEv633ToHIUIkWCE0ao7Vd/m1Iupn7QhDz0rpdzj1lytjFVqDGHo9OBXinef4OKvlit
rlVqAEzy/P3qWnGCXkRjbspDozwcvho/HUKVGLbcEj5ofJAP+5IVD2rUprzdS8AHKWe/NLY49XZo
6MCE/KVOTL56yldEXY+MOOW+rNc/ESh7Z4Xrq+j2PmrNlfo8dEfC46JW/EJE+yyn87QHRTf08yfj
Z/BVnbtcA7V5ww7j+TG1jVTTJ+6OyXby7khRHN4dC7s7oTcNy45H3kcpiNCGuCqIuHlS96V5NJqy
OkZtzt5pyJXKuZAeCydvkigwnSYlLL97m9cA8vm+qb/7CoioCKiVERjLOakDi68gdaMVXlBt+DSG
pnNFMkF1XSPiVfT8wEr1p/GTrRiRYVFmNK3q0JFk66TCjEQt2kHbvN2QxvB+Y+7GAEl4GsVsNq1h
EIuGh6GXY6afjd04ceRYBLbbx2w3jx+KyB+j/EYuRB/uDWKJgXHqpQ8esmkje18pIC+ytef5+sVf
zZMkK/oYjKIyhLv5StUiUqF9V4GYxnF8NlOjmbtmZKDzNJZXPUwrKXOK/APuATW+abIcVd8jQz3q
LOk9KLBtzVlNW3RiaPHz1QRP4K5B+y49RQM0yz+xYRBEGH37XuTqXgkRlNEoYHTxM/xqZCmzVnJD
KdovAYeWgdsj4bd0KwEezJChq/pDdmCeK2J1BlRMIIx99bR7vjr5K/79GzVm1a1lbmRzdHJlYW0K
ZW5kb2JqCjYgMCBvYmoKMjQzMAplbmRvYmoKMTQgMCBvYmoKPDwvTGVuZ3RoIDE1IDAgUi9GaWx0
ZXIgL0ZsYXRlRGVjb2RlPj4Kc3RyZWFtCnicbVPJbtswEL3rK+ZIARXDRZREoCiKAEbRNmkbhS4C
JD14oW21kZRosZN+fYcSHS8oeCDAmXnz3uPMMzDKgbnj70UZXOQprNuAwTp4DvgQBH8tSrg0mJC5
B7MKxhoOqYBUS5ppMGXAZUalBLMLyNp2VV2tGmtXddW1D4Q/hGBC8zsQgtEkwWKzxE4u197BVeFC
EXJRYBaYQ7Mxw0EmI+TWwtplMZfBlaJcjDnkP71c4kWuPdtIJoKqDPAeCqKfY/xNDaNKebB3p6X+
+Z5E0TbUVGcxl8Q2bVFX4S/z5QgEdcUKImS1V3ZPfjRF1cE25MrXQNWXc9uESJ/xOCHUg7h2VKuB
LHoaiQwdGPrmk5sQY0wmikw/55PryTdze9YaZfm+5HsF06p4gfa17WzZnopJOZWZ9taSvvpbPJ0a
IRIa++isWoItug2SPcGIBRWc7a3f4UefQQgaH3rUZ9WoJJOM++iibx7PfkLTlGu9N73s2w4s2je6
9VK03eiYGxXuBuHUOiE0ZfHBPnI5PRoZyrT2k0c+3Z7RRgzmSkcf8ese7ay10Fr0YR4iL61FSvo1
NPapbroWuhpyW1SbWbOEr6GMx4S66xebGbxvfIj+GX6PpdKHPu7sPJQeji7thzdBqWPpRjRSGmdp
oGnssDN0WAtNs/2U3l35hRHKazvYGolhjXBlii3Yg/4sRYnqePOuZ68gGE+HHrGmMd/jC/c0McEN
nn9GFwFDZW5kc3RyZWFtCmVuZG9iagoxNSAwIG9iago1NTEKZW5kb2JqCjQgMCBvYmoKPDwvVHlw
ZS9QYWdlL01lZGlhQm94IFswIDAgNTk1IDg0Ml0KL1JvdGF0ZSAwL1BhcmVudCAzIDAgUgovUmVz
b3VyY2VzPDwvUHJvY1NldFsvUERGIC9UZXh0XQovRXh0R1N0YXRlIDExIDAgUgovRm9udCAxMiAw
IFIKPj4KL0NvbnRlbnRzIDUgMCBSCj4+CmVuZG9iagoxMyAwIG9iago8PC9UeXBlL1BhZ2UvTWVk
aWFCb3ggWzAgMCA1OTUgODQyXQovUm90YXRlIDAvUGFyZW50IDMgMCBSCi9SZXNvdXJjZXM8PC9Q
cm9jU2V0Wy9QREYgL1RleHRdCi9FeHRHU3RhdGUgMTYgMCBSCi9Gb250IDE3IDAgUgo+PgovQ29u
dGVudHMgMTQgMCBSCj4+CmVuZG9iagozIDAgb2JqCjw8IC9UeXBlIC9QYWdlcyAvS2lkcyBbCjQg
MCBSCjEzIDAgUgpdIC9Db3VudCAyCj4+CmVuZG9iagoxIDAgb2JqCjw8L1R5cGUgL0NhdGFsb2cg
L1BhZ2VzIDMgMCBSCi9NZXRhZGF0YSAxOSAwIFIKPj4KZW5kb2JqCjcgMCBvYmoKPDwvVHlwZS9F
eHRHU3RhdGUKL09QTSAxPj5lbmRvYmoKMTEgMCBvYmoKPDwvUjcKNyAwIFI+PgplbmRvYmoKMTIg
MCBvYmoKPDwvUjEwCjEwIDAgUi9SOQo5IDAgUi9SOAo4IDAgUj4+CmVuZG9iagoxNiAwIG9iago8
PC9SNwo3IDAgUj4+CmVuZG9iagoxNyAwIG9iago8PC9SOQo5IDAgUi9SOAo4IDAgUj4+CmVuZG9i
agoxMCAwIG9iago8PC9CYXNlRm9udC9UaW1lcy1JdGFsaWMvVHlwZS9Gb250Ci9TdWJ0eXBlL1R5
cGUxPj4KZW5kb2JqCjkgMCBvYmoKPDwvQmFzZUZvbnQvVGltZXMtQm9sZC9UeXBlL0ZvbnQKL1N1
YnR5cGUvVHlwZTE+PgplbmRvYmoKOCAwIG9iago8PC9CYXNlRm9udC9UaW1lcy1Sb21hbi9UeXBl
L0ZvbnQKL0VuY29kaW5nIDE4IDAgUi9TdWJ0eXBlL1R5cGUxPj4KZW5kb2JqCjE4IDAgb2JqCjw8
L1R5cGUvRW5jb2RpbmcvRGlmZmVyZW5jZXNbCjE0MC9maQoxNzMvbWludXNdPj4KZW5kb2JqCjE5
IDAgb2JqCjw8L1R5cGUvTWV0YWRhdGEKL1N1YnR5cGUvWE1ML0xlbmd0aCAxMzQ0Pj5zdHJlYW0K
PD94cGFja2V0IGJlZ2luPSfvu78nIGlkPSdXNU0wTXBDZWhpSHpyZVN6TlRjemtjOWQnPz4KPD9h
ZG9iZS14YXAtZmlsdGVycyBlc2M9IkNSTEYiPz4KPHg6eG1wbWV0YSB4bWxuczp4PSdhZG9iZTpu
czptZXRhLycgeDp4bXB0az0nWE1QIHRvb2xraXQgMi45LjEtMTMsIGZyYW1ld29yayAxLjYnPgo8
cmRmOlJERiB4bWxuczpyZGY9J2h0dHA6Ly93d3cudzMub3JnLzE5OTkvMDIvMjItcmRmLXN5bnRh
eC1ucyMnIHhtbG5zOmlYPSdodHRwOi8vbnMuYWRvYmUuY29tL2lYLzEuMC8nPgo8cmRmOkRlc2Ny
aXB0aW9uIHJkZjphYm91dD0ndXVpZDo4ZmRjNjYyYi03ZjQ1LTExZjItMDAwMC0wNDI4YjJjYTYw
ODEnIHhtbG5zOnBkZj0naHR0cDovL25zLmFkb2JlLmNvbS9wZGYvMS4zLycgcGRmOlByb2R1Y2Vy
PSdHUEwgR2hvc3RzY3JpcHQgOS4wNScvPgo8cmRmOkRlc2NyaXB0aW9uIHJkZjphYm91dD0ndXVp
ZDo4ZmRjNjYyYi03ZjQ1LTExZjItMDAwMC0wNDI4YjJjYTYwODEnIHhtbG5zOnhtcD0naHR0cDov
L25zLmFkb2JlLmNvbS94YXAvMS4wLyc+PHhtcDpNb2RpZnlEYXRlPjIwMTctMDYtMDJUMDI6MTg6
MzMrMDI6MDA8L3htcDpNb2RpZnlEYXRlPgo8eG1wOkNyZWF0ZURhdGU+MjAxNy0wNi0wMlQwMjox
ODozMyswMjowMDwveG1wOkNyZWF0ZURhdGU+Cjx4bXA6Q3JlYXRvclRvb2w+Z3JvZmYgdmVyc2lv
biAxLjIxPC94bXA6Q3JlYXRvclRvb2w+PC9yZGY6RGVzY3JpcHRpb24+CjxyZGY6RGVzY3JpcHRp
b24gcmRmOmFib3V0PSd1dWlkOjhmZGM2NjJiLTdmNDUtMTFmMi0wMDAwLTA0MjhiMmNhNjA4MScg
eG1sbnM6eGFwTU09J2h0dHA6Ly9ucy5hZG9iZS5jb20veGFwLzEuMC9tbS8nIHhhcE1NOkRvY3Vt
ZW50SUQ9J3V1aWQ6OGZkYzY2MmItN2Y0NS0xMWYyLTAwMDAtMDQyOGIyY2E2MDgxJy8+CjxyZGY6
RGVzY3JpcHRpb24gcmRmOmFib3V0PSd1dWlkOjhmZGM2NjJiLTdmNDUtMTFmMi0wMDAwLTA0Mjhi
MmNhNjA4MScgeG1sbnM6ZGM9J2h0dHA6Ly9wdXJsLm9yZy9kYy9lbGVtZW50cy8xLjEvJyBkYzpm
b3JtYXQ9J2FwcGxpY2F0aW9uL3BkZic+PGRjOnRpdGxlPjxyZGY6QWx0PjxyZGY6bGkgeG1sOmxh
bmc9J3gtZGVmYXVsdCc+VW50aXRsZWQ8L3JkZjpsaT48L3JkZjpBbHQ+PC9kYzp0aXRsZT48L3Jk
ZjpEZXNjcmlwdGlvbj4KPC9yZGY6UkRGPgo8L3g6eG1wbWV0YT4KICAgICAgICAgICAgICAgICAg
ICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgCiAg
ICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAg
ICAgICAgICAgICAgIAo8P3hwYWNrZXQgZW5kPSd3Jz8+CmVuZHN0cmVhbQplbmRvYmoKMiAwIG9i
ago8PC9Qcm9kdWNlcihHUEwgR2hvc3RzY3JpcHQgOS4wNSkKL0NyZWF0aW9uRGF0ZShEOjIwMTcw
NjAyMDIxODMzKzAyJzAwJykKL01vZERhdGUoRDoyMDE3MDYwMjAyMTgzMyswMicwMCcpCi9DcmVh
dG9yKGdyb2ZmIHZlcnNpb24gMS4yMSk+PmVuZG9iagp4cmVmCjAgMjAKMDAwMDAwMDAwMCA2NTUz
NSBmIAowMDAwMDAzNTY2IDAwMDAwIG4gCjAwMDAwMDU1MjMgMDAwMDAgbiAKMDAwMDAwMzUwMCAw
MDAwMCBuIAowMDAwMDAzMTc4IDAwMDAwIG4gCjAwMDAwMDAwMTUgMDAwMDAgbiAKMDAwMDAwMjUx
NSAwMDAwMCBuIAowMDAwMDAzNjMxIDAwMDAwIG4gCjAwMDAwMDM5NTQgMDAwMDAgbiAKMDAwMDAw
Mzg4OSAwMDAwMCBuIAowMDAwMDAzODIxIDAwMDAwIG4gCjAwMDAwMDM2NzIgMDAwMDAgbiAKMDAw
MDAwMzcwMiAwMDAwMCBuIAowMDAwMDAzMzM4IDAwMDAwIG4gCjAwMDAwMDI1MzUgMDAwMDAgbiAK
MDAwMDAwMzE1OCAwMDAwMCBuIAowMDAwMDAzNzUyIDAwMDAwIG4gCjAwMDAwMDM3ODIgMDAwMDAg
biAKMDAwMDAwNDAzNiAwMDAwMCBuIAowMDAwMDA0MTAyIDAwMDAwIG4gCnRyYWlsZXIKPDwgL1Np
emUgMjAgL1Jvb3QgMSAwIFIgL0luZm8gMiAwIFIKL0lEIFs8NjZGRTlEMDdDODk2ODZGRDIxQjc3
N0E4QzVBRDBFQzI+PDY2RkU5RDA3Qzg5Njg2RkQyMUI3NzdBOEM1QUQwRUMyPl0KPj4Kc3RhcnR4
cmVmCjU2NzUKJSVFT0YK
]]

script_md5='a9e772165e8fdb620bcf9c75c17facda'
man_md5='49be4444054d85b6037d237552a7cea1'
manpdf_md5='f825d523d686dbecdc787535b40f09d0'

--> !!END-INSERTED-FILES!!

isdir=lfs.isdir
isfile=lfs.isfile
mkdir=lfs.mkdir
readdir=lfs.dir
exit=os.exit
remove=os.remove
execute=os.execute
write=io.write

kpse.set_program_name('texlua')
texdir=kpse.var_value('SELFAUTOPARENT')
bindir=kpse.var_value('SELFAUTODIR')
exedir=kpse.var_value('SELFAUTOLOC')
texmflocal=kpse.var_value('TEXMFLOCAL')

if isdir(texdir .. '/texmf/scripts') then
  texmf_dir='/texmf'
else
  texmf_dir='/texmf-dist'
end

scriptdir=texdir ..texmf_dir .. '/scripts'
instdir=texdir .. texmf_dir .. '/scripts/getnonfreefonts'
mandir=texdir .. texmf_dir .. '/doc/man/man1'
docdir=texmflocal .. '/doc/man/man1'

symlink='../..' .. texmf_dir .. '/scripts/getnonfreefonts/getnonfreefonts.pl'

local has_updmap_user=false
local exe=''; if os.type=='windows' then exe='.exe' end
if isfile (exedir..'/'..'updmap-user'..exe) then has_updmap_user=true end

--[[
print ('TEXDIR='..texdir)
print ('BINDIR='..bindir)
print ('EXEDIR='..exedir)
print ('SCRIPTDIR='..scriptdir)
print ('MANDIR='..mandir)
print ('INSTDIR='..instdir)
--]]

done  ='  [done]\n'
failed='[failed]\n'
ok    ='    [ok]\n'


if ltn12 then
  base64dec=ltn12.filter.chain(mime.decode('base64'))
end

function message (text)
  write(string.format("%-70s ", text..' ...'))
end

function detect_system ()
  -- The operating system we are currently using is derived from
  -- SELFAUTOLOC (exedir). 
  system=(string.gsub(exedir, '.*/', ''))
  if string.match(system, 'bin') then
    write ('Detected System: ' .. 'unknown '.. os.name .. '\n')
    multiplatform=false
  else
    write ('Detected System: ' .. system .. '\n')
    multiplatform=true
  end
end

function detect_installation ()
  if multiplatform then
    if isdir (scriptdir) then
      write('Detected Installation: '..texdir..'\n')
      getnonfreefonts='getnonfreefonts.pl'
    else
      write('Your TeX System seems to be broken.  Can\'t continue.\n')
      exit (1)
    end
  else
    write('Detected Installation: ' ..bindir.. 
          ' (installing in ' .. string.gsub(BINDIR,'/bin$','') .. ')\n')
    getnonfreefonts='getnonfreefonts'
    instdir=BINDIR
    mandir=MANDIR
  end
end

function md5.hex(s)
  -- Return the MD5 sum as a hexadecimal string.
  -- The argument is a string (usually the content of a file).  
  return (string.gsub(md5.sum(s), ".", 
  function (c) return string.format("%02x", string.byte(c)) end))
end


function check_md5sum (name, path, md5sum)
  -- There is a bug in older versions of Lua's MD5 library which leads
  -- to wrong checksums on 64 bit systems.  We check wether it works
  -- and skip the md5 check if necessary.  Many thanks to Aditya
  -- Mahajan for the proposal.
  if md5.hex("abcdefghijklmnopqrstuvwxyz") ==
        "c3fcd3d76192e4007dfb496cca67e13b" then
    local fh=assert(io.open(path..'/'..name, 'rb'))
    content=fh:read("*all")
    fh:close()
    local checksum=md5.hex(content)
    message ('md5sum: '..checksum..' '..name) 
    if checksum == md5sum then
      write(ok)
    else
      write(failed)
      exit(1)
    end
  end
end


function install_file (name, path, content)
  -- The argument 'content' refers to the content of the here-documents 
  mkdirhier(path)
  local file = path..'/'..name
  if multiplatform then
    message ('Installing '..file:gsub('^'..texdir..'/', ''))
  else
    message ('Installing '..file)
  end
  -- remove existing file due to bug in former release
  if isfile(file) then assert(remove(file)) end
  local fh=assert(io.open(file, 'wb'))
  fh:write(content)
  fh:close()
  write(done)
end


function check_writable (dir)
  if lfs.access then
    message ('Checking Permissions: ' .. perms)
    if lfs.access(dir, 'w') then
      write (ok)
    else
      write '\nSorry, you need admin privileges in order to continue.\n'
      exit (1)
    end
  end
end


function fix_permissions ()
  -- getnonfreefonts.pl must be executable on Unix.  We also make sure
  -- that manual pages are not executable.  Necessary if someone
  -- installed them under Windows.
  if os.type == 'unix' then
    message('Fixing File Permissions')
    execute('chmod a+x '..instdir..'/'..getnonfreefonts)
    execute('chmod a-x '..mandir..'/getnonfreefonts.1')
    write(done)
  end
end

function create_dir (dir)
  if not isdir(dir) then
    message('mkdir '..dir)
    mkdir (dir)
    if isdir(dir) then
      write(done)
    else
      write(failed)
      write("Sorry, couldn't create directory "..dir..'\n')  
      exit (1)
    end
  end
end


function mkdirhier (path)
  local dirs=string.explode(path, '/')
  for i=2, #dirs do
    local dir=table.concat(dirs, '/', 1, i)
    if not isdir(dir) then
      create_dir(dir)
    end
  end
end


-- function create_symlink (dir)
--   if os.type == 'unix' then
--     execute('cd ' .. dir ..
--             ' && ln -sf getnonfreefonts getnonfreefonts-sys')
--   end
-- end


function create_symlinks (platform, exedir)
  -- We are using shell escapes here because then we don't have to
  -- keep track of the current working directory.
  message("Creating symlink in 'bin/"..platform.."'")
  execute('cd '..exedir..' && ln -sf '..symlink..' getnonfreefonts')
  write(done)
end

function create_wrappers (platform, exedir)
  -- We don't create a new wrapper, we simply steal an existing one.
  local cp
  if os.type == 'windows' then
    exedir = exedir:gsub('/', '\\')
    cp='copy /b "'..exedir..'\\%s" "'..exedir..'\\%s"'
  else
    cp='cp -p '..exedir..'/%s '..exedir..'/%s'
  end
  if isfile(exedir..'/rungs.exe') then
    wrapper='rungs.exe';
  else -- TL 2008
    wrapper='rungs.bat';
  end
  message("Creating wrapper in 'bin/"..platform.."'")
  execute(cp:format(wrapper, 'getnonfreefonts.exe'))
  write(done)
end

function create_symlinks_and_wrappers (path)
  local otherplatforms={}
  for file in readdir(path) do
    if file ~= "." and file ~= ".." then
      local exedir = path..'/'..file
      local platform = file
      -- platform expands to something like "x86_64-linux".
      if os.type == 'unix' then
        if platform == 'win32' then
          create_wrappers (platform, exedir)
        else
          create_symlinks (platform, exedir)
        end
      else -- We're on Windows, sigh!
           -- We can't create symlinks but we can issue a warning
           -- if binaries for other platforms are available.
        if platform == 'win32' then
          create_wrappers (platform, exedir)
        else 
          otherplatforms[#otherplatforms+1]=platform
        end
        if #otherplatforms > 0 then
          write('You have binaries for Unix installed.\n' ..
                'Please run this script on Unix again in ' ..
                'order to create the symlinks.\n')
        end
      end
    end
  end
end


function texhash (dir)
  execute ('mktexlsr '..'"'..dir..'"')
end


-- main --
detect_system ()
detect_installation ()

if multiplatform then
  check_writable (scriptdir)
  create_dir (instdir) 
  docdir=mandir
else
  check_writable (instdir)
end

install_file (getnonfreefonts,            instdir, script)
install_file ('getnonfreefonts.1',        mandir,  man)


if ltn12 then
  install_file ('getnonfreefonts.man1.pdf',     docdir,  base64dec(manpdf))
end

check_md5sum (getnonfreefonts,            instdir, script_md5)
check_md5sum ('getnonfreefonts.1',        mandir,  man_md5)

if ltn12 then
  check_md5sum ('getnonfreefonts.man1.pdf',     docdir,  manpdf_md5)
end

fix_permissions ()

if multiplatform then
  create_symlinks_and_wrappers (bindir)
end
texhash (texdir..texmf_dir)


--[[
  Local Variables:
    lua-indent-level: 2
    tab-width: 2
    indent-tabs-mode: nil
  End:
  vim:set tabstop=2 expandtab:
--]]


==> install-getnonfreefonts.1 <==
#! /usr/bin/env texlua
--*- Lua -*-
--  -- pretend that this is a binary file.
-- Web browsers shall download the file, not display it.

-- Copyright (C) 2009-2015 Reinhard Kotucha <kotucha@tug.org>
--
-- You may freely use, modify and/or distribute this file.

installer_release='2018-06-04'

----------------------------------------------------------------
-- The following variables are only used for TeX systems whose
-- file system layout is not identical to that created by the
-- TeX Live installer.  This is usually the case for TeX systems
-- shipped with Linux/Unix distributions (binaries for a single 
-- platform only, and texmf* in /usr/share).
--
-- By default we install in /usr/local in order not to interfere
-- with the package manager of your Linux/Unix distribution.
--
-- These variables have no effect if you have a TeX Live system 
-- from http://texlive.org .

BINDIR='/usr/local/bin'
MANDIR='/usr/local/share/man/man1'

----------------------------------------------------------------
-- You don't have to change anything below this line.
----------------------------------------------------------------

--> !!BEGIN-INSERTED-FILES!!

-- Date: Fri Jun  2 00:18:33 2017 UTC

script=[[
#!/usr/bin/env perl

# $Id: $

# Copyright (C) 2006-2017 Reinhard Kotucha <reinhard.kotucha@web.de>
# 
# You may freely use, modify, and/or distribute this file.

my $revision='2017-06-02';

use Getopt::Long;
$Getopt::Long::autoabbrev=0;
Getopt::Long::Configure ("bundling");

my $getfont_url='https://www.tug.org/~kotucha/getnonfreefonts/getfont.pl';
my $banner="This is getnonfreefonts, revision $revision.\n\n";

# messages

my $usage = <<'ENDUSAGE';
Usage:
    getnonfreefonts --sys|--user [options] [font1] [font2] ...

    getnonfreefonts --sys installs fonts in $TEXMFLOCAL.
    getnonfreefonts --user installs fonts in $TEXMFHOME.

    In nearly all cases you should use getnonfreefonts --sys.
    For special cases see 

        http://tug.org/texlive/scripts-sys-user.html

    Options:

        -a|--all        Install all fonts.

        -d|--debug      Provide additional messages for debugging.

        -f|--force      Install fonts even if they are installed already.

        -h|--help       Print this message.

        -l|--lsfonts    List all fonts available.

        -r|--refreshmap Refresh map file.

        -H|--http       Use http instead of ftp (see manual).

        --version       Print version number.

ENDUSAGE


my $sys_user_err = <<'EOF';
ERROR: You have to invoke getnonfreefonts with either --sys or --user.

In nearly all cases you should use getnonfreefonts --sys.
For special cases see 

   http://tug.org/texlive/scripts-sys-user.html

EOF


# system specific stuff

my %sys=(
  w32     => 0,
  dirsep  => '/',
  pathsep => ':',
  exe     => '',
  dollar  => '\$',
  nulldev => '>/dev/null 2>/dev/null' 
    );

if ($^O=~/^MSWin(32|64)/i) {
  %sys=(
    w32     => 1,
    dirsep  => '\\',
    pathsep => ';',
    exe     => '.exe',
    dollar  => '$',
    nulldev => '>NUL 2>NUL' 
      );
}

# GetOptions removes optional arguments from @ARGV.
# We have to create a new array because assignments create references.

my @ARGS;
foreach my $arg (@ARGV) {
  push (@ARGS, $arg);
}

$opt_lsfonts=0;
$opt_force=0;
$opt_sys=0;
$opt_user=0;

$done=GetOptions 
    "all|a",
    "debug|d",
    "force|f",
    "help|h",
    "http|H",
    "lsfonts|l",
    "refreshmap|r",
    "verbose|v",
    "version|V",
    "sys|s",
    "user|u";

@allpackages=@ARGV;


# ANSI colors

my @supported_terminals=(
  'Eterm', 'ansi', 'color-xterm', 'con132x25', 'con132x30',
  'con132x43', 'con132x60', 'con80x25', 'con80x28', 'con80x30',
  'con80x43', 'con80x50', 'con80x60', 'cons25', 'console', 'cygwin',
  'dtterm', 'gnome', 'gnome-256color', 'konsole', 'kterm', 'linux',
  'linux-c', 'mach-color', 'mlterm', 'putty', 'rxvt', 'rxvt-cygwin',
  'rxvt-cygwin-native', 'rxvt-unicode', 'screen', 'screen-bce',
  'screen-w', 'screen.linux', 'vt100', 'xterm', 'xterm-256color',
  'xterm-color', 'xterm-debian'
    );

my $term_supported=0;

if ($ENV{'TERM'}) {
  foreach my $terminal (@supported_terminals) {
    if ($ENV{'TERM'} eq $terminal) {
      $term_supported=1;
    }
  }
}

sub colored {
  my $text=shift;
  my $color=shift;

  my $esc="\e[";
  my $restore="\e[0m";

  %colors=(
    red   => '00;31m',
    green => '00;32m'
      );

  if ($term_supported and -t 'STDOUT') {
    return "${esc}$colors{$color}${text}${restore}";
  } else {
    return $text;
  }
}

# messages

my $msglen=0;

sub msg {
  my $message=shift;
  $msglen=length($message);
  print $message;
}

sub status {
  my $status=shift;
  my $color=shift;

  
  my $spaces=79-2-$msglen-length($status);
  $spaces=1 if ($spaces < 1);
  print ' ' x $spaces;
  print ('[' . colored($status, $color) . "]\n");
}

sub debug_msg {
  my $message=shift;
  if ($opt_debug) {
    print STDERR "DEBUG: $message\n";
  }
}

# kpathsea stuff

sub var_value {
  my $var=shift;
  my $ret;

  $ret=`kpsewhich --var-value=$var`;
  chomp($ret);
  return $ret;
}

sub expand_var {
  my $var=shift;
  my $ret;
  my $dollar=$sys{'dollar'};
  $ret=`kpsewhich --expand-var=$dollar$var`;
  chomp($ret);
  return $ret;
}

sub expand_braces {
  my $var=shift;
  my $pathsep;
  my $retstring;
  my @retlist;
  if ($sys{'w32'}) {
    open KPSEWHICH, 'kpsewhich --expand-braces=$'  . "$var |";
    $pathsep=';';
  } else {
    open KPSEWHICH, 'kpsewhich --expand-braces=\$' . "$var |";
    $pathsep=':';
  }
  $retstring=(<KPSEWHICH>);
  close KPSEWHICH;
  chop $retstring;
  @retlist=split $pathsep, $retstring;
  if ($opt_debug) {
    my $index=0;
    foreach my $entry (@retlist) {
	    debug_msg "$var\[$index\]: '$entry'.";
	    ++$index;
    }
    debug_msg "Extracting the first element of the list ($var\[0\]):";
    debug_msg "$var\[0\]='$retlist[0]'.";
  }
  return "$retlist[0]";
}

sub get_tmpdir {
  if ($opt_debug) {
    for my $var (qw(TMPDIR TEMP)) {
      if (defined $ENV{$var}) {
        debug_msg "Environment variable $var='$ENV{$var}'.";
      } else {
        debug_msg "Environment variable $var not set.";
      }
    }
  }
  # get TMPDIR|TEMP environment variable, use /tmp as fallback.

  my $SYSTMP=undef;
  $SYSTMP||=$ENV{'TMPDIR'};
  $SYSTMP||=$ENV{'TEMP'};
  $SYSTMP||='/tmp';
  return "$SYSTMP";
}

sub which {
  my $prog=shift;
  my @PATH;
  my $PATH=$ENV{'PATH'};
  if ($sys{'w32'}) {
    my @PATHEXT=split ';', $ENV{'PATHEXT'};
    push @PATHEXT, '';  # if argument contains an extension
    @PATH=split ';', $PATH;
    for my $dir (@PATH) {
      $dir=~s/\\/\//g;
      for my $ext (@PATHEXT) {
        if (-f "$dir/$prog$ext") {
          return "$dir/$prog$ext";
        }
      }
    }
  } else {
    @PATH=split ':', $PATH;
    for my $dir (@PATH) {
      if (-x "$dir/$prog") {
        return "$dir/$prog";
      }
    }
  }
  return 0;
}

sub show_path {
  my @PATH;
  @PATH=split($sys{'pathsep'}, $ENV{'PATH'});
  my $index=0;
  
  foreach my $dir (@PATH) {
    debug_msg "PATH\[$index\]: '$dir'.";
    ++$index;
  }
}

sub signals {
  # Signals supposed to be supported by Windows are derived from the
  # sources of the Microsoft C runtime library.  It's a matter of fact
  # that not everything described there really works.  Furthermore,
  # the behavior depends heavily on the version of Windows you are
  # using.  Don't expect too much.
  my @signals;
  my @common_signals=qw(INT ILL FPE SEGV TERM ABRT);
  my @signals_UNIX=qw(QUIT BUS PIPE);
  my @signals_Win32=qw(BREAK);

  if ($sys{'w32'}) {
    @signals=(@common_signals, @signals_Win32);
  } else {
    @signals=(@common_signals, @signals_UNIX);
  }
  return @signals;
}


sub check_tmpdir{
  my $SYSTMP=shift;
  die "! ERROR: The temporary directory '$SYSTMP' doesn't exist.\n"
      unless (-d "$SYSTMP");

  die "! ERROR: The temporary directory '$SYSTMP' is not writable.\n"
      unless (-w "$SYSTMP");
}

sub check_installroot {
  my ($INSTALLROOTNAME, $INSTALLROOT)=@_;
  mkdir "$INSTALLROOT" unless (-d "$INSTALLROOT");

  die "! ERROR: The variable $INSTALLROOTNAME is not set.\n"
      unless length ("$INSTALLROOT") > 0;
  
  die "! ERROR: The install directory '$INSTALLROOT' doesn't " .
      "exist.\n" .
      "         If this is the correct path, please create " .
      "this directory manually.\n" 
      unless (-d "$INSTALLROOT");
  
  die "! ERROR: The install directory '$INSTALLROOT' is not writable.\n"
      unless (-w "$INSTALLROOT");
}

sub check_binary {
  my $binary=shift;
  if ($opt_debug) {
    debug_msg "Search for $binary in PATH:";
    my $binary=which "$binary";
    debug_msg "Found '$binary'.";
  }
}


### main ####

debug_msg "getnonfreefonts rev. $revision.";

debug_msg ("argv[0]: '$0'");
my $nargs=@ARGS+0;
for (0..$#ARGS) {
  my $i=$_;
  my $arg=$ARGS[$i];
  $i++;
  debug_msg ("argv[$i]: '$arg'");
}

debug_msg("opt_sys=$opt_sys");
debug_msg("opt_user=$opt_user");

show_path() if ($opt_debug);

check_binary 'kpsewhich';

# Determine INSTALLROOT.

$INSTALLROOTNAME=($opt_sys)? 'TEXMFLOCAL':'TEXMFHOME';

$INSTALLROOT=expand_braces "$INSTALLROOTNAME";

# Remove trailing exclamation marks and double slashes.

debug_msg "Removing leading \"!!\" and trailing \"//\" " . 
    "and set INSTALLROOT:";

$INSTALLROOT=~s/^!!//;
$INSTALLROOT=~s/\/\/$//;

debug_msg "INSTALLROOT='$INSTALLROOT'.";

my $SYSTMP=get_tmpdir;

debug_msg "Internal variable SYSTMP set to '$SYSTMP'.";

$^W=1 if $opt_debug;

unless ($done) {
  print STDERR "\n$banner$usage";
  exit 1;
}

if ($opt_version) {
  print "$revision\n";
  exit 0;
}

if ($opt_sys and $opt_user) {
  print STDERR "$sys_user_err";
  exit 1;
}

if ($opt_help) {
  print ($banner);
  print ($usage);

  if ($opt_sys or $opt_user) {
    print <<"ENDUSAGE";
    Directories:
       temporary: '$SYSTMP/getfont-<PID>'
       install:   '$INSTALLROOT'

ENDUSAGE
  } else {
    print "$sys_user_err";
  }
  exit 0;
}

  
unless ($opt_sys or $opt_user) {
  print "$sys_user_err";
  exit 1;
}

if ($opt_sys and $opt_user) {
  print "$sys_user_err";
  exit 1;
}


check_tmpdir $SYSTMP;
check_installroot "$INSTALLROOTNAME", "$INSTALLROOT";

my $tmpdir="$SYSTMP" . $sys{'dirsep'} . "getfont-$$";
debug_msg "Internal variable tmpdir set to '$tmpdir'.";

mkdir "$tmpdir" or die "ERROR: Can't mkdir '$tmpdir'.";
chdir "$tmpdir" or die "ERROR: Can't cd '$tmpdir'.";

#install_signal_handlers $SYSTMP, $tmpdir;

sub remove_tmpdir {
  debug_msg "Executing Signal Handler:";
  chdir "$SYSTMP" or die "! ERROR: Can't cd '$SYSTMP'.\n";
  opendir TMPDIR, "$tmpdir" 
      or print "! ERROR: Can't read directory '$tmpdir'.\n";
  my @alltmps=readdir TMPDIR;
  closedir TMPDIR;
  foreach my $file (@alltmps) {
    next if $file=~/^\./;
    unlink "$tmpdir/$file";
    debug_msg "unlink '$tmpdir/$file'.";
  }
  rmdir "$tmpdir" or die 
      "! ERROR: Can't remove directory '$tmpdir'.\n";
  debug_msg "rmdir  '$tmpdir'.";
}

foreach my $signal (signals) {
  $SIG{"$signal"}=\&remove_tmpdir;
}
debug_msg 
    "Signal handlers installed. Don't expect too much on Windows.";

my $TLROOT=expand_var 'SELFAUTOPARENT'; ### only used on Windows,
                                        ### hence no portability
                                        ### problem
my $BINDIR=expand_var 'SELFAUTOLOC';

my $has_wget=0;
my $WGET;

if ($sys{'w32'}) { ## wget is shipped with TL.
  $has_wget=1;
  if (-f "$TLROOT\\tlpkg\\installer\\wget\\wget.exe") {
    # TL-2008+
    $WGET="$TLROOT\\tlpkg\\installer\\wget\\wget.exe";
  } elsif (-f "$BINDIR\\wget.exe") {
    # TL-2005...TL-2007
    $WGET="$BINDIR\\wget.exe";
  } else {
    die "ERROR: No wget binary found.\n";
  }
} elsif (which "wget") {
  $WGET='wget';
  $has_wget=1; ## wget is in PATH.
}


debug_msg "No wget binary found on your system, trying curl." 
    unless ($has_wget);

if ($has_wget) {
  debug_msg "Running '$WGET $getfont_url'.";
  system ("$WGET", "$getfont_url") == 0 
      or die "! Error: Can't execute wget.\n";
} else {
  debug_msg "Running 'curl -O $getfont_url'.";
  system ('curl', '-O', "$getfont_url") == 0 
      or die "! Error: Can't execute curl.\n";
}

# Download the fonts.

my @getfont=('perl', "./getfont.pl");
push @getfont, "--installroot=$INSTALLROOT";
push @getfont, '--lsfonts' if $opt_lsfonts;
push @getfont, '--force' if $opt_force;
push @getfont, '--debug' if $opt_debug;
push @getfont, '--verbose' if $opt_verbose;
push @getfont, '--sys' if $opt_sys;
push @getfont, '--refreshmap' if $opt_refreshmap;
push @getfont, '--all' if $opt_all;
push @getfont, '--http' if $opt_http;
if ($has_wget) {
  push @getfont, "--wget_bin=$WGET";
} else {
  push @getfont, '--use_curl';
}
push @getfont, @allpackages;

my $getfont_cmd=join " ", @getfont;

debug_msg "Running '$getfont_cmd'.";

system @getfont;

# Evaluate the exit status.  It will be 2 if something had been
# installed and in this case we need to run texhash/updmap.

my $exit_code=$?;
my $exit_status=int($exit_code/256);

my $has_updmap_user=0;
if (-f var_value('SELFAUTOLOC').'/updmap-user'.$sys{'exe'}) {
  $has_updmap_user=1;
}

if ($opt_sys) {	     
  debug_msg "Info: Execute updmap-sys if exit status is 2.";
} else {
  if ($has_updmap_user) {
    debug_msg "Info: Execute updmap-user if exit status is 2.";
  } else {
    debug_msg "Info: Execute updmap if exit status is 2.";
  }
}

debug_msg "Exit status of getfont.pl is $exit_status.";

if ($exit_status==2) {
  print "\n";
  msg "Running 'mktexlsr $INSTALLROOT $sys{'nulldev'}' ...";
#  if ($sys{'w32'}) {
    my $ret=system "mktexlsr $INSTALLROOT $sys{'nulldev'}";
#  } else {
#    my $ret=system "mktexlsr $INSTALLROOT >/dev/null 2>/dev/null";
#  }
  
  $ret ? status 'failed', 'red' : status 'done', 'green';
   
  
  my $updmap_command;
  if ($has_updmap_user) {
    $updmap_command=($opt_sys)? 'updmap-sys':'updmap-user';
  } else {
    $updmap_command=($opt_sys)? 'updmap-sys':'updmap';
  }
  @updmap=("$updmap_command");
  push @updmap, '--quiet' unless $opt_verbose;
  print "\n";
  msg "Updating map files ($updmap_command). Be patient...";
  system @updmap;
  
  $? ? status('failed', 'red') : status('done', 'green');
}

remove_tmpdir;

__END__

# Local Variables:
#  mode: Perl
#  perl-indent-level: 2
#  indent-tabs-mode: nil
#  coding: utf-8-unix
# End:
# vim:set tabstop=2 expandtab:
]]

man=[[
.TH getnonfreefonts 1 "May 2017" "TeX Live" "TeX Live"
.SH NAME
getnonfreefonts \- download and install fonts which cannot be
distributed on a CD/DVD because the license doesn't allow to charge
money for the distribution.

.SH SYNOPSIS

.BI "getnonfreefonts --sys [" options "] [" font1 "] [" font2 "] [" font... ]
.sp
.BI "getnonfreefonts --user [" options "] [" font1 "] [" font2 "] [" font... ]

In nearly all cases you should use getnonfreefonts --sys.  For special cases see 
.br
    http://tug.org/texlive/scripts-sys-user.html
.br

.SH DESCRIPTION
Some font suppliers provide fonts which can be used freely but they
disallow that money is charged for the distribution.  Hence, for
distributions on CD or DVD it is usually impossible to include
these fonts.

.B "getnonfreefonts"
downloads and installs these fonts.

.B "getnonfreefonts --sys" 
installs files to $TEXMFLOCAL
and
.B "getnonfreefonts --user"
installs files to $TEXMFHOME

.BI "getnonfreefonts"
downloads and executes a helper script each time it is invoked.  This
script is not installed permanently on your system and only exists in
a temporary directory while
.BI "getnonfreefonts"
is running.  It allows 
.BI "getnonfreefonts"
to be aware of updates and new fonts.

Run
.B "getnonfreefonts --sys --lsfonts"
or
.B "getnonfreefonts --user --lsfonts"
to get a list of supported fonts.

.SH OPTIONS

.TP
.BR "-a" , " --all"
.rg
Install all fonts.

.TP
.BR "-d" , " --debug"
.rg
Provide additional messages for debugging.  These messages are sent to
STDERR.

.TP
.BR "-f" , " --force"
.rg
Install fonts even if they are installed already.

.TP
.BR "-h" , " --help"
.rg
Print a help message.  Nothing is installed but the directories where
the fonts will be installed and the temporary directory are shown.
.BI "<" PID ">" 
will be replaced by the process ID of the current
process. 

.TP
.BR "-H" , " --http"
.rg
Use HTTP instead of FTP.  This is useful if you are behind a firewall
which is blocking FTP.  However, you can't install fonts which are on
FTP servers.  Currently this is only "Adobe Euro".

.TP
.BR "-l" , " --lsfonts"
.rg
List all available fonts and tell whether they are installed already. 

.TP
.BR "-r" , " --refreshmap"
.rg
Register 
.B map 
files for already installed fonts and run 
.B updmap. 
This is needed after upgrading TeX Live to a newer release.

.TP
.BR "-V", " --version"
.rg
Print version number.

.SH REQUIREMENTS
On Unix systems
.BR "unzip"
and either
.BR "wget"
or 
.BR "curl"
must exist.

.SH BUGS
Please send bug reports to Reinhard Kotucha <reinhard.kotucha@web.de>.
]]

manpdf=[[
JVBERi0xLjQKJcfsj6IKNSAwIG9iago8PC9MZW5ndGggNiAwIFIvRmlsdGVyIC9GbGF0ZURlY29k
ZT4+CnN0cmVhbQp4nO1Y227cyBF911c0FgGWE3habN4ZBAEcS4YUyLYiTQIH2n2ghq0ZZilyluRI
nn/YX8k/5lQ3u3nxyKsk+xj4Qcawu7q66tSpU/0zc7lgLv3r/64fT05vYrZpT1y2Ofn5RKiPrP+z
fmR/XmFBQj+sHk70HsFij8Wpz5OUrR5PhJ9w32er5xNnI7uqrh4aKR/qqmt/cMQPC7ZarP554nku
jyJsXuU4idbKz+yqoE9L+BKy1RpreKJXkMlIm3ySbEOrXFohwpALT69xjpzVm/NESqtPb1L4zdOQ
XF/6acLDhC39SO3++HZklYep31v9cE6/D1eG34EbsyWOJde5Gx27KfsXy2vamPjci9K0vyh3w5SW
3znPVVlnOcuqnBVV22VlyfTG522x3rJ1VlV1x+4ly4u2a4r7Bc51XS9w9p3MWV2xjL07Oz1bBPRz
kDp/P8PidbZvJeu2kpXFWlatXPy4+svJ0vjQ++zktWyr71UWuA50xIPEFf2Nu8xGIuWxSFMT4LKs
R5sQSV+4/TdcqFt4oevUa3Wm2u0FPECUR0m+c7ZZsxAJd0UoEDP2WFfayd5oEPEeFM7hYUiIyxPf
+Hfn1I26o4mMSHmahBSZoq64sjbNtIgC7iPTXgI8kenbf3z8dH17easzm/aZBRD6CN3ZdC5EzNNU
pA7yusB90iQQjsrTctkeWnbXHyfc3kgacEDbgKfekU/tKGrDcZ4Obr/yxzt725E1IbiwF3cIIOK4
LZeHkcnFq215L9oawPBaW5zzaTQ9H6UxuKQq0fMED32BTASvDzMg3RyJM6IX/z/OR+M8kBUiHnM3
sRF3LitWyawpD4wYZ521smWHes/abb0vc0b0MWcyBXQ+I+Z0oN33M1IILCk4TfsCk+zkusjM+a2U
Gh1+yr1wqMFt1+3+cHra7Te8HhCyOe3kQoTOl7LQ7Gacij0epPboJzk62ksAKMMep+26KXZdS9dS
4FqgibgiiBy+7R7LY/yBIMZj/jg7v313c3m9uvz0cRrvgULQdKJYU95t/SgVubN2v9uVhWxatmtq
XEIf+1Tkck7+xPzwLWeUB2RL87+IBViOyK/nzJjOIP5O0XtjQ5z5QJxqiYlJ0WaWws1OgXzZ4gCH
H9+5zTpN1f3ehJb4gFYYm7AeioUXRzxOY6cd9wDBoyAS1k5DJmA8TGxjQKSSvofivprcFSD8JOEi
CIa+1RM+ORFy36JeYQ/7dQNgF7Jayze0Kkx4NOk+ZH3SUGNf72qppb47Y/iueyolBj216FjRIhN7
RO7Aisdd3bbFfYkmW6Nvr8t9rvpt2ydw3H0UdNB6U/Lz9YzXWzCIihIe235yh9aNLtuLh3asHtpv
umGsfNsN2hQkPAhMYKEbhE7NwARTwGN5FIbpsFxh3rFO/VKiwBGr363OP394f/Xp3dsr8npKYQLu
uX5o7jj1zfeO+zZuD1OfQrRg1zeYnruikRWhomPLNY527+KTEXuWXBGuq5PV7/+rvKVJYvqT1oLg
wHCO+XEq5YRkwxgq1FbOlxf4zFlDEGI728pyh0apyY3JDDzSFSAejeCiMlJYC1xSosbCU23O1db7
unR+Gh/p+/bIngDgfM7ZalsoSPg+1GA03E7JXKf3Bg6Qmu1TIXOdA6RT+MFAmAE8ok24xmNWyapD
xaEq0Z5wrUPbyUcVpbrC78o1EUGC+oE5NAj1hPAFBU43RlCwZ1c3WXNA1Tdy3dX4Hzi2lDMABjGP
DB+9AECVa6jMY7lGN4x9S7Ks2VdVUW1Uz6QCSUyBOJeKYJcB6CtJxdDqFC9TYbezykXLGXjuf2QP
PWahGNFbsnHKIf/DoWk/D/If8mMkdxrJ6ge23+WZQhxSYRqCwmuCtA965nmk3qFQwlHR8l4LoppH
yuRmX82Sgqjayen1iny5LFv9IfXiYzGhbu5bf5rZodNJ41eRYPTpr5/qe9ygACmAYcCzBFIppqQL
6qZT7c8EaDasIkdeKEYa5JOSHy+OMM4ym7IizeSua2r7zXSfCcdyCSTO5l0Pc7pVCJf9rGrn1Zka
pWl68HGZz31IRsx13Ic7OJHLUXvezCIJhwSh1RbPtdFSYaq1VJbnBTV1KMxH2bbZBnBVnR9myRY0
Bb0mTLXDZkMlCz5DFyXHIggXi31dOtZYhlJoQVDU2W5XZ+c3N/MweIHHvXQciodpKCKybgjzG6EA
qPqr9Ro4gTBZy3lMAkXQNvmXkyeFWV8JuLDiq9fJfQnPlHIFSRekBHznoRskHcb3ZBDa2xcNOIcJ
k6T+wLCIn20GwFIjs/ywiIwMn6sXgcFgAqvtfw4rhJI65FfYHkMJ3SQMtVC8boqq67uqARFfLEM/
BFWGzse62wIuurOae+iXCKp/rdFtzykkKXvZ6KeZXukXSM/9JAyQRQqdHmkOAX2imyztOdbHFAi3
9eJ7xS1+Yvm7mk+I0Pg233/U3+yECVrpv1xfns1l2Shnzp+mocNN40SYpmdu08hdma0pFgd1V4w5
awSPXZ4RzdEv633ToHIUIkWCE0ao7Vd/m1Iupn7QhDz0rpdzj1lytjFVqDGHo9OBXinef4OKvlit
rlVqAEzy/P3qWnGCXkRjbspDozwcvho/HUKVGLbcEj5ofJAP+5IVD2rUprzdS8AHKWe/NLY49XZo
6MCE/KVOTL56yldEXY+MOOW+rNc/ESh7Z4Xrq+j2PmrNlfo8dEfC46JW/EJE+yyn87QHRTf08yfj
Z/BVnbtcA7V5ww7j+TG1jVTTJ+6OyXby7khRHN4dC7s7oTcNy45H3kcpiNCGuCqIuHlS96V5NJqy
OkZtzt5pyJXKuZAeCydvkigwnSYlLL97m9cA8vm+qb/7CoioCKiVERjLOakDi68gdaMVXlBt+DSG
pnNFMkF1XSPiVfT8wEr1p/GTrRiRYVFmNK3q0JFk66TCjEQt2kHbvN2QxvB+Y+7GAEl4GsVsNq1h
EIuGh6GXY6afjd04ceRYBLbbx2w3jx+KyB+j/EYuRB/uDWKJgXHqpQ8esmkje18pIC+ytef5+sVf
zZMkK/oYjKIyhLv5StUiUqF9V4GYxnF8NlOjmbtmZKDzNJZXPUwrKXOK/APuATW+abIcVd8jQz3q
LOk9KLBtzVlNW3RiaPHz1QRP4K5B+y49RQM0yz+xYRBEGH37XuTqXgkRlNEoYHTxM/xqZCmzVnJD
KdovAYeWgdsj4bd0KwEezJChq/pDdmCeK2J1BlRMIIx99bR7vjr5K/79GzVm1a1lbmRzdHJlYW0K
ZW5kb2JqCjYgMCBvYmoKMjQzMAplbmRvYmoKMTQgMCBvYmoKPDwvTGVuZ3RoIDE1IDAgUi9GaWx0
ZXIgL0ZsYXRlRGVjb2RlPj4Kc3RyZWFtCnicbVPJbtswEL3rK+ZIARXDRZREoCiKAEbRNmkbhS4C
JD14oW21kZRosZN+fYcSHS8oeCDAmXnz3uPMMzDKgbnj70UZXOQprNuAwTp4DvgQBH8tSrg0mJC5
B7MKxhoOqYBUS5ppMGXAZUalBLMLyNp2VV2tGmtXddW1D4Q/hGBC8zsQgtEkwWKzxE4u197BVeFC
EXJRYBaYQ7Mxw0EmI+TWwtplMZfBlaJcjDnkP71c4kWuPdtIJoKqDPAeCqKfY/xNDaNKebB3p6X+
+Z5E0TbUVGcxl8Q2bVFX4S/z5QgEdcUKImS1V3ZPfjRF1cE25MrXQNWXc9uESJ/xOCHUg7h2VKuB
LHoaiQwdGPrmk5sQY0wmikw/55PryTdze9YaZfm+5HsF06p4gfa17WzZnopJOZWZ9taSvvpbPJ0a
IRIa++isWoItug2SPcGIBRWc7a3f4UefQQgaH3rUZ9WoJJOM++iibx7PfkLTlGu9N73s2w4s2je6
9VK03eiYGxXuBuHUOiE0ZfHBPnI5PRoZyrT2k0c+3Z7RRgzmSkcf8ese7ay10Fr0YR4iL61FSvo1
NPapbroWuhpyW1SbWbOEr6GMx4S66xebGbxvfIj+GX6PpdKHPu7sPJQeji7thzdBqWPpRjRSGmdp
oGnssDN0WAtNs/2U3l35hRHKazvYGolhjXBlii3Yg/4sRYnqePOuZ68gGE+HHrGmMd/jC/c0McEN
nn9GFwFDZW5kc3RyZWFtCmVuZG9iagoxNSAwIG9iago1NTEKZW5kb2JqCjQgMCBvYmoKPDwvVHlw
ZS9QYWdlL01lZGlhQm94IFswIDAgNTk1IDg0Ml0KL1JvdGF0ZSAwL1BhcmVudCAzIDAgUgovUmVz
b3VyY2VzPDwvUHJvY1NldFsvUERGIC9UZXh0XQovRXh0R1N0YXRlIDExIDAgUgovRm9udCAxMiAw
IFIKPj4KL0NvbnRlbnRzIDUgMCBSCj4+CmVuZG9iagoxMyAwIG9iago8PC9UeXBlL1BhZ2UvTWVk
aWFCb3ggWzAgMCA1OTUgODQyXQovUm90YXRlIDAvUGFyZW50IDMgMCBSCi9SZXNvdXJjZXM8PC9Q
cm9jU2V0Wy9QREYgL1RleHRdCi9FeHRHU3RhdGUgMTYgMCBSCi9Gb250IDE3IDAgUgo+PgovQ29u
dGVudHMgMTQgMCBSCj4+CmVuZG9iagozIDAgb2JqCjw8IC9UeXBlIC9QYWdlcyAvS2lkcyBbCjQg
MCBSCjEzIDAgUgpdIC9Db3VudCAyCj4+CmVuZG9iagoxIDAgb2JqCjw8L1R5cGUgL0NhdGFsb2cg
L1BhZ2VzIDMgMCBSCi9NZXRhZGF0YSAxOSAwIFIKPj4KZW5kb2JqCjcgMCBvYmoKPDwvVHlwZS9F
eHRHU3RhdGUKL09QTSAxPj5lbmRvYmoKMTEgMCBvYmoKPDwvUjcKNyAwIFI+PgplbmRvYmoKMTIg
MCBvYmoKPDwvUjEwCjEwIDAgUi9SOQo5IDAgUi9SOAo4IDAgUj4+CmVuZG9iagoxNiAwIG9iago8
PC9SNwo3IDAgUj4+CmVuZG9iagoxNyAwIG9iago8PC9SOQo5IDAgUi9SOAo4IDAgUj4+CmVuZG9i
agoxMCAwIG9iago8PC9CYXNlRm9udC9UaW1lcy1JdGFsaWMvVHlwZS9Gb250Ci9TdWJ0eXBlL1R5
cGUxPj4KZW5kb2JqCjkgMCBvYmoKPDwvQmFzZUZvbnQvVGltZXMtQm9sZC9UeXBlL0ZvbnQKL1N1
YnR5cGUvVHlwZTE+PgplbmRvYmoKOCAwIG9iago8PC9CYXNlRm9udC9UaW1lcy1Sb21hbi9UeXBl
L0ZvbnQKL0VuY29kaW5nIDE4IDAgUi9TdWJ0eXBlL1R5cGUxPj4KZW5kb2JqCjE4IDAgb2JqCjw8
L1R5cGUvRW5jb2RpbmcvRGlmZmVyZW5jZXNbCjE0MC9maQoxNzMvbWludXNdPj4KZW5kb2JqCjE5
IDAgb2JqCjw8L1R5cGUvTWV0YWRhdGEKL1N1YnR5cGUvWE1ML0xlbmd0aCAxMzQ0Pj5zdHJlYW0K
PD94cGFja2V0IGJlZ2luPSfvu78nIGlkPSdXNU0wTXBDZWhpSHpyZVN6TlRjemtjOWQnPz4KPD9h
ZG9iZS14YXAtZmlsdGVycyBlc2M9IkNSTEYiPz4KPHg6eG1wbWV0YSB4bWxuczp4PSdhZG9iZTpu
czptZXRhLycgeDp4bXB0az0nWE1QIHRvb2xraXQgMi45LjEtMTMsIGZyYW1ld29yayAxLjYnPgo8
cmRmOlJERiB4bWxuczpyZGY9J2h0dHA6Ly93d3cudzMub3JnLzE5OTkvMDIvMjItcmRmLXN5bnRh
eC1ucyMnIHhtbG5zOmlYPSdodHRwOi8vbnMuYWRvYmUuY29tL2lYLzEuMC8nPgo8cmRmOkRlc2Ny
aXB0aW9uIHJkZjphYm91dD0ndXVpZDo4ZmRjNjYyYi03ZjQ1LTExZjItMDAwMC0wNDI4YjJjYTYw
ODEnIHhtbG5zOnBkZj0naHR0cDovL25zLmFkb2JlLmNvbS9wZGYvMS4zLycgcGRmOlByb2R1Y2Vy
PSdHUEwgR2hvc3RzY3JpcHQgOS4wNScvPgo8cmRmOkRlc2NyaXB0aW9uIHJkZjphYm91dD0ndXVp
ZDo4ZmRjNjYyYi03ZjQ1LTExZjItMDAwMC0wNDI4YjJjYTYwODEnIHhtbG5zOnhtcD0naHR0cDov
L25zLmFkb2JlLmNvbS94YXAvMS4wLyc+PHhtcDpNb2RpZnlEYXRlPjIwMTctMDYtMDJUMDI6MTg6
MzMrMDI6MDA8L3htcDpNb2RpZnlEYXRlPgo8eG1wOkNyZWF0ZURhdGU+MjAxNy0wNi0wMlQwMjox
ODozMyswMjowMDwveG1wOkNyZWF0ZURhdGU+Cjx4bXA6Q3JlYXRvclRvb2w+Z3JvZmYgdmVyc2lv
biAxLjIxPC94bXA6Q3JlYXRvclRvb2w+PC9yZGY6RGVzY3JpcHRpb24+CjxyZGY6RGVzY3JpcHRp
b24gcmRmOmFib3V0PSd1dWlkOjhmZGM2NjJiLTdmNDUtMTFmMi0wMDAwLTA0MjhiMmNhNjA4MScg
eG1sbnM6eGFwTU09J2h0dHA6Ly9ucy5hZG9iZS5jb20veGFwLzEuMC9tbS8nIHhhcE1NOkRvY3Vt
ZW50SUQ9J3V1aWQ6OGZkYzY2MmItN2Y0NS0xMWYyLTAwMDAtMDQyOGIyY2E2MDgxJy8+CjxyZGY6
RGVzY3JpcHRpb24gcmRmOmFib3V0PSd1dWlkOjhmZGM2NjJiLTdmNDUtMTFmMi0wMDAwLTA0Mjhi
MmNhNjA4MScgeG1sbnM6ZGM9J2h0dHA6Ly9wdXJsLm9yZy9kYy9lbGVtZW50cy8xLjEvJyBkYzpm
b3JtYXQ9J2FwcGxpY2F0aW9uL3BkZic+PGRjOnRpdGxlPjxyZGY6QWx0PjxyZGY6bGkgeG1sOmxh
bmc9J3gtZGVmYXVsdCc+VW50aXRsZWQ8L3JkZjpsaT48L3JkZjpBbHQ+PC9kYzp0aXRsZT48L3Jk
ZjpEZXNjcmlwdGlvbj4KPC9yZGY6UkRGPgo8L3g6eG1wbWV0YT4KICAgICAgICAgICAgICAgICAg
ICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgCiAg
ICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAgICAg
ICAgICAgICAgICAgIAo8P3hwYWNrZXQgZW5kPSd3Jz8+CmVuZHN0cmVhbQplbmRvYmoKMiAwIG9i
ago8PC9Qcm9kdWNlcihHUEwgR2hvc3RzY3JpcHQgOS4wNSkKL0NyZWF0aW9uRGF0ZShEOjIwMTcw
NjAyMDIxODMzKzAyJzAwJykKL01vZERhdGUoRDoyMDE3MDYwMjAyMTgzMyswMicwMCcpCi9DcmVh
dG9yKGdyb2ZmIHZlcnNpb24gMS4yMSk+PmVuZG9iagp4cmVmCjAgMjAKMDAwMDAwMDAwMCA2NTUz
NSBmIAowMDAwMDAzNTY2IDAwMDAwIG4gCjAwMDAwMDU1MjMgMDAwMDAgbiAKMDAwMDAwMzUwMCAw
MDAwMCBuIAowMDAwMDAzMTc4IDAwMDAwIG4gCjAwMDAwMDAwMTUgMDAwMDAgbiAKMDAwMDAwMjUx
NSAwMDAwMCBuIAowMDAwMDAzNjMxIDAwMDAwIG4gCjAwMDAwMDM5NTQgMDAwMDAgbiAKMDAwMDAw
Mzg4OSAwMDAwMCBuIAowMDAwMDAzODIxIDAwMDAwIG4gCjAwMDAwMDM2NzIgMDAwMDAgbiAKMDAw
MDAwMzcwMiAwMDAwMCBuIAowMDAwMDAzMzM4IDAwMDAwIG4gCjAwMDAwMDI1MzUgMDAwMDAgbiAK
MDAwMDAwMzE1OCAwMDAwMCBuIAowMDAwMDAzNzUyIDAwMDAwIG4gCjAwMDAwMDM3ODIgMDAwMDAg
biAKMDAwMDAwNDAzNiAwMDAwMCBuIAowMDAwMDA0MTAyIDAwMDAwIG4gCnRyYWlsZXIKPDwgL1Np
emUgMjAgL1Jvb3QgMSAwIFIgL0luZm8gMiAwIFIKL0lEIFs8NjZGRTlEMDdDODk2ODZGRDIxQjc3
N0E4QzVBRDBFQzI+PDY2RkU5RDA3Qzg5Njg2RkQyMUI3NzdBOEM1QUQwRUMyPl0KPj4Kc3RhcnR4
cmVmCjU2NzUKJSVFT0YK
]]

script_md5='a9e772165e8fdb620bcf9c75c17facda'
man_md5='49be4444054d85b6037d237552a7cea1'
manpdf_md5='f825d523d686dbecdc787535b40f09d0'

--> !!END-INSERTED-FILES!!

isdir=lfs.isdir
isfile=lfs.isfile
mkdir=lfs.mkdir
readdir=lfs.dir
exit=os.exit
remove=os.remove
execute=os.execute
write=io.write

kpse.set_program_name('texlua')
texdir=kpse.var_value('SELFAUTOPARENT')
bindir=kpse.var_value('SELFAUTODIR')
exedir=kpse.var_value('SELFAUTOLOC')
texmflocal=kpse.var_value('TEXMFLOCAL')

if isdir(texdir .. '/texmf/scripts') then
  texmf_dir='/texmf'
else
  texmf_dir='/texmf-dist'
end

scriptdir=texdir ..texmf_dir .. '/scripts'
instdir=texdir .. texmf_dir .. '/scripts/getnonfreefonts'
mandir=texdir .. texmf_dir .. '/doc/man/man1'
docdir=texmflocal .. '/doc/man/man1'

symlink='../..' .. texmf_dir .. '/scripts/getnonfreefonts/getnonfreefonts.pl'

local has_updmap_user=false
local exe=''; if os.type=='windows' then exe='.exe' end
if isfile (exedir..'/'..'updmap-user'..exe) then has_updmap_user=true end

--[[
print ('TEXDIR='..texdir)
print ('BINDIR='..bindir)
print ('EXEDIR='..exedir)
print ('SCRIPTDIR='..scriptdir)
print ('MANDIR='..mandir)
print ('INSTDIR='..instdir)
--]]

done  ='  [done]\n'
failed='[failed]\n'
ok    ='    [ok]\n'


if ltn12 then
  base64dec=ltn12.filter.chain(mime.decode('base64'))
end

function message (text)
  write(string.format("%-70s ", text..' ...'))
end

function detect_system ()
  -- The operating system we are currently using is derived from
  -- SELFAUTOLOC (exedir). 
  system=(string.gsub(exedir, '.*/', ''))
  if string.match(system, 'bin') then
    write ('Detected System: ' .. 'unknown '.. os.name .. '\n')
    multiplatform=false
  else
    write ('Detected System: ' .. system .. '\n')
    multiplatform=true
  end
end

function detect_installation ()
  if multiplatform then
    if isdir (scriptdir) then
      write('Detected Installation: '..texdir..'\n')
      getnonfreefonts='getnonfreefonts.pl'
    else
      write('Your TeX System seems to be broken.  Can\'t continue.\n')
      exit (1)
    end
  else
    write('Detected Installation: ' ..bindir.. 
          ' (installing in ' .. string.gsub(BINDIR,'/bin$','') .. ')\n')
    getnonfreefonts='getnonfreefonts'
    instdir=BINDIR
    mandir=MANDIR
  end
end

function md5.hex(s)
  -- Return the MD5 sum as a hexadecimal string.
  -- The argument is a string (usually the content of a file).  
  return (string.gsub(md5.sum(s), ".", 
  function (c) return string.format("%02x", string.byte(c)) end))
end


function check_md5sum (name, path, md5sum)
  -- There is a bug in older versions of Lua's MD5 library which leads
  -- to wrong checksums on 64 bit systems.  We check wether it works
  -- and skip the md5 check if necessary.  Many thanks to Aditya
  -- Mahajan for the proposal.
  if md5.hex("abcdefghijklmnopqrstuvwxyz") ==
        "c3fcd3d76192e4007dfb496cca67e13b" then
    local fh=assert(io.open(path..'/'..name, 'rb'))
    content=fh:read("*all")
    fh:close()
    local checksum=md5.hex(content)
    message ('md5sum: '..checksum..' '..name) 
    if checksum == md5sum then
      write(ok)
    else
      write(failed)
      exit(1)
    end
  end
end


function install_file (name, path, content)
  -- The argument 'content' refers to the content of the here-documents 
  mkdirhier(path)
  local file = path..'/'..name
  if multiplatform then
    message ('Installing '..file:gsub('^'..texdir..'/', ''))
  else
    message ('Installing '..file)
  end
  -- remove existing file due to bug in former release
  if isfile(file) then assert(remove(file)) end
  local fh=assert(io.open(file, 'wb'))
  fh:write(content)
  fh:close()
  write(done)
end


function check_writable (dir)
  if lfs.access then
    message ('Checking Permissions: ' .. perms)
    if lfs.access(dir, 'w') then
      write (ok)
    else
      write '\nSorry, you need admin privileges in order to continue.\n'
      exit (1)
    end
  end
end


function fix_permissions ()
  -- getnonfreefonts.pl must be executable on Unix.  We also make sure
  -- that manual pages are not executable.  Necessary if someone
  -- installed them under Windows.
  if os.type == 'unix' then
    message('Fixing File Permissions')
    execute('chmod a+x '..instdir..'/'..getnonfreefonts)
    execute('chmod a-x '..mandir..'/getnonfreefonts.1')
    write(done)
  end
end

function create_dir (dir)
  if not isdir(dir) then
    message('mkdir '..dir)
    mkdir (dir)
    if isdir(dir) then
      write(done)
    else
      write(failed)
      write("Sorry, couldn't create directory "..dir..'\n')  
      exit (1)
    end
  end
end


function mkdirhier (path)
  local dirs=string.explode(path, '/')
  for i=2, #dirs do
    local dir=table.concat(dirs, '/', 1, i)
    if not isdir(dir) then
      create_dir(dir)
    end
  end
end


-- function create_symlink (dir)
--   if os.type == 'unix' then
--     execute('cd ' .. dir ..
--             ' && ln -sf getnonfreefonts getnonfreefonts-sys')
--   end
-- end


function create_symlinks (platform, exedir)
  -- We are using shell escapes here because then we don't have to
  -- keep track of the current working directory.
  message("Creating symlink in 'bin/"..platform.."'")
  execute('cd '..exedir..' && ln -sf '..symlink..' getnonfreefonts')
  write(done)
end

function create_wrappers (platform, exedir)
  -- We don't create a new wrapper, we simply steal an existing one.
  local cp
  if os.type == 'windows' then
    exedir = exedir:gsub('/', '\\')
    cp='copy /b "'..exedir..'\\%s" "'..exedir..'\\%s"'
  else
    cp='cp -p '..exedir..'/%s '..exedir..'/%s'
  end
  if isfile(exedir..'/rungs.exe') then
    wrapper='rungs.exe';
  else -- TL 2008
    wrapper='rungs.bat';
  end
  message("Creating wrapper in 'bin/"..platform.."'")
  execute(cp:format(wrapper, 'getnonfreefonts.exe'))
  write(done)
end

function create_symlinks_and_wrappers (path)
  local otherplatforms={}
  for file in readdir(path) do
    if file ~= "." and file ~= ".." then
      local exedir = path..'/'..file
      local platform = file
      -- platform expands to something like "x86_64-linux".
      if os.type == 'unix' then
        if platform == 'win32' then
          create_wrappers (platform, exedir)
        else
          create_symlinks (platform, exedir)
        end
      else -- We're on Windows, sigh!
           -- We can't create symlinks but we can issue a warning
           -- if binaries for other platforms are available.
        if platform == 'win32' then
          create_wrappers (platform, exedir)
        else 
          otherplatforms[#otherplatforms+1]=platform
        end
        if #otherplatforms > 0 then
          write('You have binaries for Unix installed.\n' ..
                'Please run this script on Unix again in ' ..
                'order to create the symlinks.\n')
        end
      end
    end
  end
end


function texhash (dir)
  execute ('mktexlsr '..'"'..dir..'"')
end


-- main --
detect_system ()
detect_installation ()

if multiplatform then
  check_writable (scriptdir)
  create_dir (instdir) 
  docdir=mandir
else
  check_writable (instdir)
end

install_file (getnonfreefonts,            instdir, script)
install_file ('getnonfreefonts.1',        mandir,  man)


if ltn12 then
  install_file ('getnonfreefonts.man1.pdf',     docdir,  base64dec(manpdf))
end

check_md5sum (getnonfreefonts,            instdir, script_md5)
check_md5sum ('getnonfreefonts.1',        mandir,  man_md5)

if ltn12 then
  check_md5sum ('getnonfreefonts.man1.pdf',     docdir,  manpdf_md5)
end

fix_permissions ()

if multiplatform then
  create_symlinks_and_wrappers (bindir)
end
texhash (texdir..texmf_dir)


--[[
  Local Variables:
    lua-indent-level: 2
    tab-width: 2
    indent-tabs-mode: nil
  End:
  vim:set tabstop=2 expandtab:
--]]

